The While language

This article presents a formalisation of a simple imperative programming language. The objective is to study and develop "hands-on" a formal specifcation of a programming language, namely its syntax, operational semantics and type system. To have an executable version of the language, we implemented in Racket its operational semantics and type system.

==> useful-macros.tex <==
% Colours

\usepackage{color}
\definecolor{dkblue}{rgb}{0,0.1,0.5}
\definecolor{dkgreen}{rgb}{0,0.4,0}
\def\Red{\color{\ifdraft red\else black\fi}}
\def\Green{\color{\ifdraft green\else black\fi}}
\def\Blue{\color{\ifdraft blue\else black\fi}}
\def\Black{\color{black}}
\newcommand{\details}[1]{\iffull{\Blue#1}\fi}
\definecolor{linkColor}{rgb}{0,0,0.5}

% Theorems etc.
\makeatletter
\@ifclassloaded{beamer}
  {\relax}
  {\newtheorem{theorem}{Theorem}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}

\newtheorem{saetning}{S{\ae}tning}
\newtheorem{proposition}{Proposition}
\newtheorem{korollar}{Korollar}

\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{eksempel}{Eksempel}
\newtheorem{exercise}{Exercise}
\newtheorem{problem}[theorem]{Problem}}
\makeatother
\newenvironment{bevis}{\begin{proof}[Bevis:]}{\end{proof}}

\input{commands}

==> useful-packages.tex <==
% Common packages

\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{listings}
\usepackage{xspace}
\usepackage{graphicx}
\usepackage{stmaryrd}
\usepackage{tikz}

